The Robots are Here: Navigating the Generative AI Revolution in Computing Education

Recent advancements in artificial intelligence (AI) are fundamentally reshaping computing, with large language models (LLMs) now effectively being able to generate and interpret source code and natural language instructions. These emergent capabilities have sparked urgent questions in the computing education community around how educators should adapt their pedagogy to address the challenges and to leverage the opportunities presented by this new technology. In this working group report, we undertake a comprehensive exploration of LLMs in the context of computing education and make five significant contributions. First, we provide a detailed review of the literature on LLMs in computing education and synthesise findings from 71 primary articles. Second, we report the findings of a survey of computing students and instructors from across 20 countries, capturing prevailing attitudes towards LLMs and their use in computing education contexts. Third, to understand how pedagogy is already changing, we offer insights collected from in-depth interviews with 22 computing educators from five continents who have already adapted their curricula and assessments. Fourth, we use the ACM Code of Ethics to frame a discussion of ethical issues raised by the use of large language models in computing education, and we provide concrete advice for policy makers, educators, and students. Finally, we benchmark the performance of LLMs on various computing education datasets, and highlight the extent to which the capabilities of current models are rapidly improving. Our aim is that this report will serve as a focal point for both researchers and practitioners who are exploring, adapting, using, and evaluating LLMs and LLM-based tools in computing classrooms.

==> appendices/instructor-guide.tex <==
\section{Guide for instructions}

==> temp.tex <==
\section{Review of Literature}

% Intro ... goals of this section
The working group aimed to identify prior work that explores how \LLMS might impact computing education. We used the work we found to inform the other activities of the working group, but we also present a summary of this work as a snapshot of the quickly evolving literature in this area and 

\subsection{Method}

We chose to perform a scoping review to rapidly identify gaps and major themes in the work. We explicitly considered but decided not to perform a systematic review, as the research in this area is evolving quickly and relies heavily on dissemination through non-traditional publication channels such as arXiv. We chose to perform one step of forward and backward snowballing from a set of reference papers that were identified as being currently significant work in the area of \LLMS in computing education.

\input{tables/reference_papers}

The reference papers were initially identified by the working group leaders, who have published in the area, as being influential. Then, the papers were discussed by the full working group reach a consensus on inclusion. During the discussion, concerns about the scope of venues were raised, so work from outside SIGCSE-sponsored venues was explicitly added to identify a broader set of literature. The resulting set, listed in Table~\ref{tab:ref-papers}, includes 10 papers. By necessity due to the age of the research area, these papers are largely published in 2022 and 2023. 

Each paper that cites or is cited by at least one of the reference papers was evaluated for inclusion by two working group members. During this review, the paper was not read in detail; rather, the evaluator searched for evidence that it should be given deeper consideration. As a result, .... papers were evaluated using the criteria below.

\begin{enumerate}
\item \textit{Must have direct applicability to computing education.} This criterion was refined to the following and was interpreted generously:
  \begin{enumerate}
      \item The paper explicitly states a relation to computing education, 
      \item the participants include students working on problems typical of a computing education context,
      \item the problems or inputs featured are drawn from a computing education context, OR
      \item the resource or tool being created is dspecifically designed for computing education.
  \end{enumerate}
  \item \textit{Must mention generative AI, \LLMS, or a specific tool using those technologies, such as Copilot.}
  \item \textit{At least 4 pages in length (inclusive).} This criterion rules out posters and extended abstracts.
  \item \textit{Written in English.}
  \item \textit{"Published" in or after 2021.} For papers published in non-traditional venues such as arXiv, this is the upload date.
\end{enumerate}

Each of the five major criteria had to be satisfied to include the paper. Each paper was independently evaluated twice; the evaluator could flag the paper for inclusion, exclusion, or discussion. If there was disagreement between the two evaluators or if they flagged the paper for discussion, it was evaluated by a third evaluator who made a final decision. As a result, papers were included if (a) both initial evaluators flagged it for inclusion or (b) if at least one evaluator flagged it for inclusion or discussion and the third evaluator agreed that it should be included. All evaluators were instructed to interpret the criteria generously, to avoid exclusion of potentially relevant work. After these reviews, ... (...\%) papers were identified for inclusion. 

\input{tables/paper_extraction}

Finally, each of the papers selected for inclusion were read in depth by a single member of the working team. The goal of this step was to . In addition, we extracted some details about the type of work being performed, such as evidence of research quality. Data extraction was guided by a set of questions implemented as an online form. The questions on the form are presented in~\table{tab:paper-extraction}.

During this final step, ...  papers were flagged as not being relevant. The exclusion of some papers at this stage was expected, as the reviewers had been instructed to identify any \textit{potentially} relevant work. These exclusions left us with ... relevant papers (including the original ten reference papers) which are presented below.

\subsection{Themes}

% Subsubsections for each theme.
